Human-Machine Co-Boosted Bug Report Identification with Mutualistic Neural Active Learning

Bug reports, encompassing a wide range of bug types, are crucial for maintaining software quality. However, the increasing complexity and volume of bug reports pose a significant challenge in sole manual identification and assignment to the appropriate teams for resolution, as dealing with all the reports is time-consuming and resource-intensive. In this paper, we introduce a cross-project framework, dubbed Mutualistic Neural Active Learning (MNAL), designed for automated and more effective identification of bug reports from GitHub repositories boosted by human-machine collaboration. MNAL utilizes a neural language model that learns and generalizes reports across different projects, coupled with active learning to form neural active learning. A distinctive feature of MNAL is the purposely crafted mutualistic relation between the machine learners (neural language model) and human labelers (developers) when enriching the knowledge learned. That is, the most informative human-labeled reports and their corresponding pseudo-labeled ones are used to update the model while those reports that need to be labeled by developers are more readable and identifiable, thereby enhancing the human-machine teaming therein. We evaluate MNAL using a large scale dataset against the SOTA approaches, baselines, and different variants. The results indicate that MNAL achieves up to 95.8% and 196.0% effort reduction in terms of readability and identifiability during human labeling, respectively, while resulting in a better performance in bug report identification. Additionally, our MNAL is model-agnostic since it is capable of improving the model performance with various underlying neural language models. To further verify the efficacy of our approach, we conducted a qualitative case study involving 10 human participants, who rate MNAL as being more effective while saving more time and monetary resources.

==> tab/fig15.tex <==
% \begin{table}[t!]
% 	\centering
%         \footnotesize
% 	\setlength{\tabcolsep}{2mm}
% 	\caption{RQ1: Mean (SD) values of metrics comparing among different active learning strategies. The best value of each performance indicator is in \textcolor{red}{RED}.}
% 	\label{tab:rq1-1}%
% 	%\begin{threeparttable}
% 	\begin{tabular}{ccccccccc}\toprule
% 	\textbf{Step size}&\textbf{Methods/Metrics}\hspace{-0.5cm}&\textbf{F1-score}&\textbf{Accuracy}&\textbf{Recall}&\textbf{Precision}&\textbf{Readability}&\textbf{Identifiability}\\\midrule % times 27
  	
%    \multirow{3}{*}{300} &Random&0.858&0.851&0.848&0.869&-54.075&0.053\\
%    &Uncertainty&\textcolor{red}{0.87}&\textcolor{red}{0.862}&\textcolor{red}{0.87}&\textcolor{red}{0.87}&-37.361&0.037\\
%    &Effort&0.862&0.852&0.868&0.857&\textcolor{red}{14.894}&\textcolor{red}{0.153}\\
% \midrule
%    \multirow{3}{*}{500} &Random&0.868&0.86&0.866&0.871&-49.1&0.053\\
%    &Uncertainty&\textcolor{red}{0.874}&\textcolor{red}{0.866}&0.873&\textcolor{red}{0.875}&-41.326&0.039\\
%    &Effort&0.872&0.863&\textcolor{red}{0.878}&0.867&\textcolor{red}{-15.404}&\textcolor{red}{0.098}\\
% \midrule
%    \multirow{3}{*}{700} &Random&0.861&0.861&0.866&0.871&-53.58&0.053\\
%    &Uncertainty&\textcolor{red}{0.878}&\textcolor{red}{0.87}&0.878&\textcolor{red}{0.878}&-36.44&0.04\\
%    &Effort&0.878&0.869&\textcolor{red}{0.883}&0.873&\textcolor{red}{-11.354}&\textcolor{red}{0.093}\\
%     \bottomrule
% 	\end{tabular}	
% \end{table}%

\begin{table}[t!]
	\centering
        \footnotesize
	\setlength{\tabcolsep}{0.8mm}
	\caption{Different pseudo labeling ratio comparison for F1 scores, readability and identifiability on 10 runs. $r$ denotes the rank produced by Scott-Knott test and the statistically best results are highlighted in \setlength{\fboxsep}{1.5pt}\colorbox{teal!20}{green}.}
	\label{tab:rq1-1}%
% \resizebox{\textwidth}{!}{ % reSize the table
\begin{adjustbox}{width=\textwidth}
% \begin{tabular}{p{0.4cm}p{1.2cm}p{0.1cm}p{1.3cm}|p{0.1cm}p{1.3cm}|p{0.1cm}p{1.3cm}|p{0.1cm}p{1.3cm}|p{0.1cm}p{1.3cm}|p{0.1cm}p{1.3cm}}
\begin{tabular}{ll|llllllll|llllll}
\toprule
 \multirow{2}{*}{\textbf{Query size}} &
  \multirow{2}{*}{\textbf{Ratio}} &
  \multicolumn{2}{c}{\textbf{F1-score}} &
  \multicolumn{2}{c}{\textbf{Accuracy}} &
  \multicolumn{2}{c}{\textbf{Recall}} &
  \multicolumn{2}{c|}{\textbf{Precision}}&
  \multicolumn{2}{c}{\textbf{Readability}} &
  \multicolumn{2}{c}{\textbf{Identifiability}}\\ \cline{3-14}

 &
   &
  \textbf{$r$} &
  \textbf{Mean (SD)} &
  \textbf{$r$} &
  \textbf{Mean (SD)} &
  \textbf{$r$} &
  \textbf{Mean (SD)} &
  \textbf{$r$} &
  \textbf{Mean (SD)} &
  \textbf{$r$} &
  \textbf{Mean (SD)} &
  \textbf{$r$} &
  \textbf{Mean (SD)} \\ \midrule
%  &
%   \texttt{\approach$_{ran}$}  &3&0.858&3&0.851&3&0.848&1&\textcolor{red}{0.869}&3&-54.075&2&0.053\\
%  &
%   \texttt{\approach$_{un}$} &1&\textcolor{red}{0.87}&1&\textcolor{red}{0.862}&1&\textcolor{red}{0.87}&1&\textcolor{red}{0.87}&2&-37.361&3&0.037 \\
% \multirow{-3}{*}{300} &
%   \texttt{\approach} &2&0.864&2&0.853&2&0.873&2&0.855&1&\textcolor{red}{8.074}&1&\textcolor{red}{0.129} \\  \hline
  
%  &
%   \texttt{\approach$_{ran}$}  &3&0.868&3&0.86&3&0.866&2&0.871&3&-49.1&2&0.053\\
%  &
%   \texttt{\approach$_{un}$} &1&\textcolor{red}{0.874}&1&\textcolor{red}{0.866}&2&0.873&1&\textcolor{red}{0.875}&2&-41.326&3&0.039 \\
% \multirow{-3}{*}{500} &
%   \texttt{\approach} &2&0.872&2&0.863&1&0.878&3&0.867&1&\textcolor{red}{-15.404}&1&\textcolor{red}{0.098} \\  \hline
  
%  &
%   \texttt{\approach$_{ran}$}  &2&0.861&3&0.861&3&0.866&3&0.871&3&-53.58&2&0.053\\
%  &
%   \texttt{\approach$_{un}$} &1&\textcolor{red}{0.878}&1&\textcolor{red}{0.87}&2&0.878&1&\textcolor{red}{0.878}&2&-36.44&3&0.04 \\
% \multirow{-3}{*}{700} &
%   \texttt{\approach} &1&\textcolor{red}{0.878}&2&0.869&1&\textcolor{red}{0.883}&2&0.873&1&\textcolor{red}{-11.354}&1&\textcolor{red}{0.093}\\\bottomrule
 &
  \textbf{1}&1&0.855 ($\pm 0.018$)&1&0.847 ($\pm 0.017$)&2&0.852 ($\pm 0.031$)&1&0.859 ($\pm 0.016$)&1&1.77 ($\pm 36.207$)&1&0.167 ($\pm 0.104$)\\
 &
  \textbf{2}&1&0.856 ($\pm 0.015$)&1&0.847 ($\pm 0.015$)&2&0.856 ($\pm 0.025$)&1&0.856 ($\pm 0.015$)&1&0.447 ($\pm 38.644$)&1&0.176 ($\pm 0.119$)\\
\multirow{-3}{*}{300} &
  \textbf{3}&1&0.858 ($\pm 0.016$)&1&0.849 ($\pm 0.015$)&\cellcolor{teal!20}1&\cellcolor{teal!20}0.861 ($\pm 0.028$)&1&0.856 ($\pm 0.015$)&1&3.119 ($\pm 23.335$)&1&0.162 ($\pm 0.113$)\\  \hline
  
 &
  \textbf{1}&1&0.864 ($\pm 0.015$)&1&0.856 ($\pm 0.014$)&2&0.863 ($\pm 0.026$)&\cellcolor{teal!20}1&\cellcolor{teal!20}0.865 ($\pm 0.01$)&\cellcolor{teal!20}1&\cellcolor{teal!20}-2.511 ($\pm 18.956$)&1&0.145 ($\pm 0.106$)\\
 &
  \textbf{2}&1&0.866 ($\pm 0.013$)&1&0.857 ($\pm 0.012$)&\cellcolor{teal!20}1&\cellcolor{teal!20}0.869 ($\pm 0.021$)&\cellcolor{teal!20}1&\cellcolor{teal!20}0.864 ($\pm 0.009$)&\cellcolor{teal!20}1&\cellcolor{teal!20}-6.369 ($\pm 21.299$)&1&0.138 ($\pm 0.103$)\\
\multirow{-3}{*}{500} &
  \textbf{3}&1&0.866 ($\pm 0.012$)&1&0.856 ($\pm 0.012$)&\cellcolor{teal!20}1&\cellcolor{teal!20}0.869 ($\pm 0.019$)&2&0.862 ($\pm 0.011$)&2&-11.14 ($\pm 22.775$)&1&0.13 ($\pm 0.091$)\\  \hline
  
 &
  \textbf{1}&2&0.869 ($\pm 0.011$)&2&0.861 ($\pm 0.011$)&2&0.871 ($\pm 0.019$)&1&0.868 ($\pm 0.009$)&1&-10.555 ($\pm 18.465$)&1&0.132 ($\pm 0.1$)\\
 &
  \textbf{2}&\cellcolor{teal!20}1&\cellcolor{teal!20}0.872 ($\pm 0.011$)&\cellcolor{teal!20}1&\cellcolor{teal!20}0.863 ($\pm 0.011$)&\cellcolor{teal!20}1&\cellcolor{teal!20}0.876 ($\pm 0.019$)&1&0.868 ($\pm 0.009$)&1&-13.744 ($\pm 17.741$)&1&0.127 ($\pm 0.096$)\\
\multirow{-3}{*}{700} &
  \textbf{3}&2&0.869 ($\pm 0.011$)&2&0.86 ($\pm 0.01$)&2&0.873 ($\pm 0.018$)&1&0.866 ($\pm 0.01$)&1&-12.845 ($\pm 16.071$)&1&0.124 ($\pm 0.093$)\\  \hline


\end{tabular}
\end{adjustbox}
\end{table}%


==> tab/rq1.tex <==
\begin{table}[t!]
	\centering
        \footnotesize
	\setlength{\tabcolsep}{2mm}
	\caption{RQ1: Scott-Knott rank of metrics comparing for different active learning strategies. }
	\label{tab:rq1-1}%
	%\begin{threeparttable}
	\begin{tabular}{ccccccccc}\toprule
	\textbf{Step size}&\textbf{Methods/Metrics}\hspace{-0.5cm}&\textbf{F1-score}&\textbf{Accuracy}&\textbf{Recall}&\textbf{Precision}&\textbf{Readability}&\textbf{Identifiability}\\\midrule % times 27
  	
   \multirow{3}{*}{300} &Random&3&3&3&1&3&2\\
   &Uncertainty&1&1&1&1&2&3\\
   &Effort&2&2&2&2&1&1\\
\midrule
   \multirow{3}{*}{500} &Random&3&3&3&2&3&2\\
   &Uncertainty&1&1&2&3&2&3\\
   &Effort&2&2&1&1&1&1\\
\midrule
   \multirow{3}{*}{700} &Random&2&3&3&3&3&2\\
   &Uncertainty&1&1&2&1&2&3\\
   &Effort&1&2&1&2&1&1\\
	\end{tabular}	
\end{table}%

==> tab/rq1_med.tex <==
\begin{table}[t!]
	\centering
        \footnotesize
	\setlength{\tabcolsep}{2mm}
	\caption{RQ1: Median values of metrics comparing among different active learning strategies. The best value of each performance indicator is in \textcolor{red}{RED}.}
	\label{tab:rq1-1}%
	%\begin{threeparttable}
	\begin{tabular}{ccccccccc}\toprule
	\textbf{Step size}&\textbf{Methods/Metrics}\hspace{-0.5cm}&\textbf{F1-score}&\textbf{Accuracy}&\textbf{AUC}&\textbf{Recall}&\textbf{Precision}&\textbf{Readability}&\textbf{Identifiability}\\\midrule % times 27
  	
   \multirow{3}{*}{300} &Random&0.86&0.853&0.913&0.849&0.87&-53.693&0.053\\
   &Uncertainty&0.869&0.861&0.916&0.872&0.872&-37.933&0.037\\
   &Effort&0.861&0.852&0.914&0.864&0.856&11.82&0.131\\
\midrule
   \multirow{3}{*}{500} &Random&0.868&0.859&0.912&0.868&0.87&-53.166&0.054\\
   &Uncertainty&0.874&0.865&0.915&0.873&0.874&-39.95&0.038\\
   &Effort&0.873&0.864&0.916&0.884&0.867&-5.026&0.096\\
\midrule
   \multirow{3}{*}{700} &Random&0.868&0.86&0.917&0.863&0.872&-50.818&0.054\\
   &Uncertainty&0.879&0.871&0.918&0.877&0.879&-38.777&0.04\\
   &Effort&0.879&0.87&0.923&0.885&0.871&-12.964&0.087\\
    \bottomrule
	\end{tabular}	
\end{table}%

==> tab/rq2.tex <==
\begin{table}[t!]
	\centering
        \footnotesize
	\setlength{\tabcolsep}{2mm}
	\caption{RQ2: Scott-Knott rank of metrics between using pseudo-labeling and without using pseudo-labeling. }
	\label{tab:rq1-1}%
	%\begin{threeparttable}
	\begin{tabular}{ccccccccc}\toprule
	\textbf{Step size}&\textbf{Methods/Metrics}\hspace{-0.5cm}&\textbf{F1-score}&\textbf{Accuracy}&\textbf{Recall}&\textbf{Precision}&\textbf{Readability}&\textbf{Identifiability}\\\midrule % times 27
  	
   \multirow{3}{*}{300} &With Pseudo-labeling&1&1&1&1&2&2\\
   &W/O Pseudo-labeling&2&2&2&2&1&1\\
\midrule
   \multirow{3}{*}{500} &With Pseudo-labeling&1&1&1&1&1&2\\
   &W/O Pseudo-labeling&2&2&2&2&1&1\\
\midrule
   \multirow{3}{*}{700} &With Pseudo-labeling&1&1&1&1&1&1\\
   &W/O Pseudo-labeling&2&2&2&1&1&2\\
	\end{tabular}	
\end{table}%

==> tab/rq2_avg.tex <==

% \begin{table}[t!]
% 	\centering
% 	\setlength{\tabcolsep}{2mm}
% 	\caption{RQ2: Average values of metrics comparing between using pseudo-labeling and without using pseudo-labeling. The best value of each performance indicator is in \textcolor{red}{RED}.}
% 	\label{tab:rq2-1}%
% 	%\begin{threeparttable}
%     \footnotesize
% 	\begin{tabular}{ccccccccc}\toprule
% 	\textbf{Step size}&\textbf{Methods/Metrics}\hspace{-0.5cm}&\textbf{F1-score}&\textbf{Accuracy}&\textbf{Recall}&\textbf{Precision}&\textbf{Readability}&\textbf{Identifiability}\\\midrule % times 27

%    \multirow{2}{*}{300} &With Pseudo-labeling&\textcolor{red}{0.871}&\textcolor{red}{0.862}&\textcolor{red}{0.877}&\textcolor{red}{0.866}&-2.131&0.098\\
%    &W/O Pseudo-labeling&0.862&0.852&0.868&0.857&\textcolor{red}{14.894}&\textcolor{red}{0.153}\\
% \midrule
%    \multirow{2}{*}{500} &With Pseudo-labeling&\textcolor{red}{0.878}&\textcolor{red}{0.869}&\textcolor{red}{0.883}&\textcolor{red}{0.873}&\textcolor{red}{-14.226}&0.089\\
%    &W/O Pseudo-labeling&0.872&0.863&0.878&0.867&-15.404&\textcolor{red}{0.098}\\
% \midrule
%    \multirow{2}{*}{700} &With Pseudo-labeling&\textcolor{red}{0.880}&\textcolor{red}{0.871}&\textcolor{red}{0.887}&0.873&-13.21&\textcolor{red}{0.118}\\
%    &W/O Pseudo-labeling&0.878&0.869&0.883&\textcolor{red}{0.873}&\textcolor{red}{-11.354}&0.093\\

%     \bottomrule
% 	\end{tabular}
% \end{table}%

% \begin{table}[t!]
% 	\centering
% 	\setlength{\tabcolsep}{2mm}
% 	\caption{RQ2: Average values of metrics at the final step  comparing between using pseudo-labeling and without using pseudo-labeling. The best value of each performance indicator is in green.}
% \resizebox{\textwidth}{!}{ % reSize the table
% \begin{tabular}{p{0.7cm}p{3.5cm}p{0.3cm}p{1.55cm}|p{0.3cm}p{1.55cm}|p{0.3cm}p{1.4cm}|p{0.3cm}p{1.4cm}|p{0.3cm}p{1.55cm}|p{0.3cm}p{1.4cm}}
% \toprule
%  &
%   \multirow{2}{*}{\textbf{Approach}} &
%   \multicolumn{2}{c}{\textsc{\textbf{F1-score}}} &
%   \multicolumn{2}{c}{\textsc{\textbf{Accuracy}}} &
%   \multicolumn{2}{c}{\textsc{\textbf{Recall}}} &
%   \multicolumn{2}{c}{\textsc{\textbf{Precision}}} &
%   \multicolumn{2}{c}{\textsc{\textbf{Readability}}} &
%   \multicolumn{2}{c}{\textsc{\textbf{Identifiability}}}\\ \cline{3-14}

%  &
%    &
%   \textbf{$r$} &
%   \textbf{Average} &
%   \textbf{$r$} &
%   \textbf{Average} &
%   \textbf{$r$} &
%   \textbf{Average} &
%   \textbf{$r$} &
%   \textbf{Average} &
%   \textbf{$r$} &
%   \textbf{Average} &
%   \textbf{$r$} &
%   \textbf{Average} \\ \hline
%  &
%   \texttt{w/o pseduo labeling}  &2&0.864&2&0.853&\cellcolor{teal!20}1&\cellcolor{teal!20}0.873&2&0.855&\cellcolor{teal!20}1&\cellcolor{teal!20}8.074&\cellcolor{teal!20}1&\cellcolor{teal!20}0.129\\
% \multirow{-2}{*}{300} &
%   \texttt{with pseudo-labeling} &\cellcolor{teal!20}1&\cellcolor{teal!20}0.87&\cellcolor{teal!20}1&\cellcolor{teal!20}0.861&2&0.872&\cellcolor{teal!20}1&\cellcolor{teal!20}0.868&2&6.779&2&0.115 \\ \hline
  
%  &
%   \texttt{w/o pseduo labeling}  &2&0.872&2&0.863&2&0.878&2&0.867&2&-15.404&\cellcolor{teal!20}1&\cellcolor{teal!20}0.098\\
% \multirow{-2}{*}{500} &
%   \texttt{with pseudo-labeling} &\cellcolor{teal!20}1&\cellcolor{teal!20}0.877&\cellcolor{teal!20}1&\cellcolor{teal!20}0.868&\cellcolor{teal!20}1&\cellcolor{teal!20}0.883&\cellcolor{teal!20}1&\cellcolor{teal!20}0.87&\cellcolor{teal!20}1&\cellcolor{teal!20}-8.392&2&0.09 \\ \hline
  
%  &
%   \texttt{w/o pseduo labeling}  &2&0.878&2&0.869&2&0.883&1&0.873&1&-11.354&1&0.093\\
% \multirow{-2}{*}{700} &
%   \texttt{with pseudo-labeling} &\cellcolor{teal!20}1&\cellcolor{teal!20}0.880&\cellcolor{teal!20}1&\cellcolor{teal!20}0.871&\cellcolor{teal!20}1&\cellcolor{teal!20}0.887&1&0.873&1&-10.246&1&0.094\\\bottomrule

% %  &
% %   \texttt{w/o pseduo labeling}  &2&0.85&2&0.841&1&0.848&2&0.852&\cellcolor{teal!20}1&\cellcolor{teal!20}5.75&1&0.188\\
% % \multirow{-2}{*}{300} &
% %   \texttt{with pseudo-labeling} &\cellcolor{teal!20}1&\cellcolor{teal!20}0.855&\cellcolor{teal!20}1&\cellcolor{teal!20}0.847&1&0.852&\cellcolor{teal!20}1&\cellcolor{teal!20}0.859&2&1.071&1&0.155\\ \hline
  
% %  &
% %   \texttt{w/o pseduo labeling}  &2&0.861&2&0.853&1&0.861&2&0.862&\cellcolor{teal!20}1&\cellcolor{teal!20}-0.119&1&0.143\\
% % \multirow{-2}{*}{500} &
% %   \texttt{with pseudo-labeling} &\cellcolor{teal!20}1&\cellcolor{teal!20}0.864&\cellcolor{teal!20}1&\cellcolor{teal!20}0.856&1&0.863&\cellcolor{teal!20}1&\cellcolor{teal!20}0.865&2&-1.671&1&0.136\\ \hline
  
% %  &
% %   \texttt{w/o pseduo labeling}  &1&0.867&1&0.859&1&0.869&2&0.867&\cellcolor{teal!20}1&\cellcolor{teal!20}-8.617&1&0.134\\
% % \multirow{-2}{*}{700} &
% %   \texttt{with pseudo-labeling} &1&0.869&1&0.861&1&0.871&\cellcolor{teal!20}1&\cellcolor{teal!20}0.868&2&-9.53&1&0.122\\\bottomrule
% \end{tabular}
% }
% \end{table}%

\begin{table}[t!]
	\centering
	\setlength{\tabcolsep}{2mm}
	\caption{RQ2: Average values of metrics over ten steps comparing between using pseudo-labeling and without using pseudo-labeling. The best value of each performance indicator is in green.}
\resizebox{\textwidth}{!}{ % reSize the table
\begin{tabular}{l{0.7cm}l{3.5cm}l{0.3cm}l{1.55cm}|l{0.3cm}l{1.55cm}|l{0.3cm}l{1.4cm}|l{0.3cm}l{1.4cm}|l{0.3cm}l{1.55cm}|l{0.3cm}l{1.4cm}}
\toprule
 &
  \multirow{2}{*}{\textbf{Approach}} &
  \multicolumn{2}{c}{\textbf{F1-score}} &
  \multicolumn{2}{c}{\textbf{Accuracy}} &
  \multicolumn{2}{c}{\textbf{Recall}} &
  \multicolumn{2}{c}{\textbf{Precision}} &
  \multicolumn{2}{c}{\textbf{Readability}} &
  \multicolumn{2}{c}{\textbf{Identifiability}}\\ \cline{3-14}

 &
   &
  \textbf{$r$} &
  \textbf{Average} &
  \textbf{$r$} &
  \textbf{Average} &
  \textbf{$r$} &
  \textbf{Average} &
  \textbf{$r$} &
  \textbf{Average} &
  \textbf{$r$} &
  \textbf{Average} &
  \textbf{$r$} &
  \textbf{Average} \\ \hline
%  &
%   \texttt{w/o pseduo labeling}  &2&0.864&2&0.853&\cellcolor{teal!20}1&\cellcolor{teal!20}0.873&2&0.855&\cellcolor{teal!20}1&\cellcolor{teal!20}8.074&\cellcolor{teal!20}1&\cellcolor{teal!20}0.129\\
% \multirow{-2}{*}{300} &
%   \texttt{with pseudo-labeling} &\cellcolor{teal!20}1&\cellcolor{teal!20}0.87&\cellcolor{teal!20}1&\cellcolor{teal!20}0.861&2&0.872&\cellcolor{teal!20}1&\cellcolor{teal!20}0.868&2&6.779&2&0.115 \\ \hline
  
%  &
%   \texttt{w/o pseduo labeling}  &2&0.872&2&0.863&2&0.878&2&0.867&2&-15.404&\cellcolor{teal!20}1&\cellcolor{teal!20}0.098\\
% \multirow{-2}{*}{500} &
%   \texttt{with pseudo-labeling} &\cellcolor{teal!20}1&\cellcolor{teal!20}0.877&\cellcolor{teal!20}1&\cellcolor{teal!20}0.868&\cellcolor{teal!20}1&\cellcolor{teal!20}0.883&\cellcolor{teal!20}1&\cellcolor{teal!20}0.87&\cellcolor{teal!20}1&\cellcolor{teal!20}-8.392&2&0.09 \\ \hline
  
%  &
%   \texttt{w/o pseduo labeling}  &2&0.878&2&0.869&2&0.883&1&0.873&1&-11.354&1&0.093\\
% \multirow{-2}{*}{700} &
%   \texttt{with pseudo-labeling} &\cellcolor{teal!20}1&\cellcolor{teal!20}0.880&\cellcolor{teal!20}1&\cellcolor{teal!20}0.871&\cellcolor{teal!20}1&\cellcolor{teal!20}0.887&1&0.873&1&-10.246&1&0.094\\\bottomrule

 &
  \texttt{w/o pseduo labeling}  &2&0.85&2&0.841&1&0.848&2&0.852&1&5.75&1&0.188\\
\multirow{-2}{*}{300} &
  \texttt{with pseudo-labeling} &\cellcolor{teal!20}1&\cellcolor{teal!20}0.855&\cellcolor{teal!20}1&\cellcolor{teal!20}0.847&1&0.852&\cellcolor{teal!20}1&\cellcolor{teal!20}0.859&1&1.071&1&0.155\\ \hline
  
 &
  \texttt{w/o pseduo labeling}  &1&0.861&2&0.853&1&0.861&2&0.862&1&-0.119&1&0.143\\
\multirow{-2}{*}{500} &
  \texttt{with pseudo-labeling} &1&0.864&\cellcolor{teal!20}1&\cellcolor{teal!20}0.856&1&0.863&\cellcolor{teal!20}1&\cellcolor{teal!20}0.865&1&-1.671&1&0.136\\ \hline
  
 &
  \texttt{w/o pseduo labeling}  &1&0.867&1&0.859&1&0.869&1&0.867&1&-8.617&1&0.134\\
\multirow{-2}{*}{700} &
  \texttt{with pseudo-labeling} &1&0.869&1&0.861&1&0.871&1&0.868&1&-9.53&1&0.122\\\bottomrule
\end{tabular}
}
\end{table}%


==> tab/rq2_med.tex <==

\begin{table}[t!]
	\centering
	\setlength{\tabcolsep}{2mm}
	\caption{RQ2: Median values of metrics comparing between using pseudo-labeling and without using pseudo-labeling. The best value of each performance indicator is in \textcolor{red}{RED}.}
	\label{tab:rq2-1}%
	%\begin{threeparttable}
    \footnotesize
	\begin{tabular}{ccccccccc}\toprule
	\textbf{Step size}&\textbf{Methods/Metrics}\hspace{-0.5cm}&\textbf{F1-score}&\textbf{Accuracy}&\textbf{AUC}&\textbf{Recall}&\textbf{Precision}&\textbf{Readability}&\textbf{Identifiability}\\\midrule % times 27

   \multirow{2}{*}{300} &With Pseudo-labeling&0.872&0.862&0.918&0.877&0.865&-3.491&0.098\\
   &W/O Pseudo-labeling&0.873&0.864&0.916&0.884&0.867&-5.026&0.096\\
\midrule
   \multirow{2}{*}{500} &With Pseudo-labeling&0.878&0.87&0.916&0.883&0.872&-14.705&0.089\\
   &W/O Pseudo-labeling&0.873&0.864&0.916&0.884&0.867&-5.026&0.096\\
\midrule   
   \multirow{2}{*}{700} &With Pseudo-labeling&0.879&0.87&0.919&0.886&0.873&-12.524&0.094\\
   &W/O Pseudo-labeling&0.879&0.87&0.923&0.885&0.871&-12.964&0.087\\

    \bottomrule
	\end{tabular}
\end{table}%

==> tab/rq3.tex <==
\begin{table}[t!]
	\centering
	\setlength{\tabcolsep}{2mm}
	\caption{RQ3: Scott-Knott rank of metrics between random and our method when using different pretrained language models.}

	% \label{tab:rq3-1}%
	%\begin{threeparttable}
    \footnotesize
	\begin{tabular}{cccccccccc}\toprule
	\textbf{Step size}&\textbf{Model}&\textbf{Methods}\hspace{-0.5cm}&\textbf{F1-score}&\textbf{Accuracy}&\textbf{Recall}&\textbf{Precision}&\textbf{Readability}&\textbf{Identifiability}\\\midrule % times 27

   \multirow{6}{*}{300}&\multirow{2}{*}{CodeBERT}&Random&2&2&2&2&2&2\\
   &&\approach&1&1&1&1&1&1\\\cmidrule{2-10}
   &\multirow{2}{*}{RoBERTa}&Random&2&2&2&2&2&2\\
   &&\approach&1&1&1&1&1&1\\\cmidrule{2-10}
   &\multirow{2}{*}{RTA}&Random&2&2&2&1&2&2\\
   &&\approach&1&1&1&2&1&1\\
\midrule
   \multirow{6}{*}{500}&\multirow{2}{*}{CodeBERT}&Random&2&2&2&1&2&2\\
   &&\approach&1&1&1&1&1&1\\\cmidrule{2-10}
   &\multirow{2}{*}{RoBERTa}&Random&2&2&2&2&2&2\\
   &&\approach&1&1&1&1&1&1\\\cmidrule{2-10}
   &\multirow{2}{*}{RTA}&Random&2&2&2&1&2&2\\
   &&\approach&1&1&1&1&1&1\\
\midrule
   \multirow{6}{*}{700}&\multirow{2}{*}{CodeBERT}&Random&2&2&2&1&2&2\\
   &&\approach&1&1&1&1&1&1\\\cmidrule{2-10}
   &\multirow{2}{*}{RoBERTa}&Random&2&2&2&2&2&2\\
   &&\approach&1&1&1&1&1&1\\\cmidrule{2-10}
   &\multirow{2}{*}{RTA}&Random&2&2&2&1&2&2\\
   &&\approach&1&1&&1&1&1&1\\
    \bottomrule
	\end{tabular}

\label{tab:rq3-1}
\end{table}%

==> tab/rq3_avg.tex <==
% \begin{table}[t!]
% 	\centering
% 	\setlength{\tabcolsep}{2mm}
% 	\caption{RQ3: Average values of metrics comparing between \approach$_{ran}$ and our method when using different pretrained language models. The best value of each performance indicator is in \textcolor{red}{RED}.}

% 	% \label{tab:rq3-1}%
% 	%\begin{threeparttable}
%     \footnotesize
% 	\begin{tabular}{cccccccccc}\toprule
% 	\textbf{Step size}&\textbf{Model}&\textbf{Methods}\hspace{-0.5cm}&\textbf{F1-score}&\textbf{Accuracy}&\textbf{Recall}&\textbf{Precision}&\textbf{Readability}&\textbf{Identifiability}\\\midrule % times 27

%    \multirow{6}{*}{300}&\multirow{2}{*}{CodeBERT}&\approach$_{ran}$&0.864&0.856&0.862&0.867&-49.548&0.053\\
%    &&\approach&\textcolor{red}{0.875}&\textcolor{red}{0.866}&\textcolor{red}{0.881}&\textcolor{red}{0.87}&\textcolor{red}{-13.376}&\textcolor{red}{0.113}\\\cmidrule{2-10}
%    &\multirow{2}{*}{RoBERTa}&\approach$_{ran}$&0.867&0.857&0.87&0.863&-59.287&0.052\\
%    &&\approach&\textcolor{red}{0.877}&\textcolor{red}{0.867}&\textcolor{red}{0.885}&\textcolor{red}{0.868}&\textcolor{red}{-6.543}&\textcolor{red}{0.101}\\\cmidrule{2-10}
%    &\multirow{2}{*}{RTA}&\approach$_{ran}$&0.879&0.871&0.883&\textcolor{red}{0.875}&-54.043&0.052\\
%    &&\approach&\textcolor{red}{0.886}&\textcolor{red}{0.877}&\textcolor{red}{0.897}&0.874&\textcolor{red}{-2.207}&\textcolor{red}{0.108}\\
% \midrule
%    \multirow{6}{*}{500}&\multirow{2}{*}{CodeBERT}&\approach$_{ran}$&0.869&0.861&0.867&0.872&-47.712&0.054\\
%    &&\approach&\textcolor{red}{0.88}&\textcolor{red}{0.871}&\textcolor{red}{0.887}&\textcolor{red}{0.873}&\textcolor{red}{-13.942}&\textcolor{red}{0.087}\\\cmidrule{2-10}
%    &\multirow{2}{*}{RoBERTa}&\approach$_{ran}$&0.87&0.861&0.869&0.87&-50.123&0.053\\
%    &&\approach&\textcolor{red}{0.88}&\textcolor{red}{0.871}&\textcolor{red}{0.888}&\textcolor{red}{0.872}&\textcolor{red}{-11.754}&\textcolor{red}{0.103}\\\cmidrule{2-10}
%    &\multirow{2}{*}{RTA}&\approach$_{ran}$&0.884&0.875&0.89&0.878&-56.962&0.053\\
%    &&\approach&\textcolor{red}{0.889}&\textcolor{red}{0.881}&\textcolor{red}{0.9}&\textcolor{red}{0.879}&\textcolor{red}{-11.52}&\textcolor{red}{0.129}\\
% \midrule
%    \multirow{6}{*}{700}&\multirow{2}{*}{CodeBERT}&\approach$_{ran}$&0.872&0.864&0.871&0.873&-57.184&0.052\\
%    &&\approach&\textcolor{red}{0.882}&\textcolor{red}{0.873}&\textcolor{red}{0.889}&\textcolor{red}{0.874}&\textcolor{red}{-14.614}&\textcolor{red}{0.135}\\\cmidrule{2-10}
%    &\multirow{2}{*}{RoBERTa}&\approach$_{ran}$&0.871&0.862&0.872&0.87&-47.866&0.053\\
%    &&\approach&\textcolor{red}{0.882}&\textcolor{red}{0.873}&\textcolor{red}{0.89}&\textcolor{red}{0.874}&\textcolor{red}{-15.198}&\textcolor{red}{0.117}\\\cmidrule{2-10}
%    &\multirow{2}{*}{RTA}&\approach$_{ran}$&0.884&0.876&0.889&0.879&-51.048&0.053\\
%    &&\approach&\textcolor{red}{0.889}&\textcolor{red}{0.881}&&\textcolor{red}{0.9}&0.879&\textcolor{red}{-14.105}&\textcolor{red}{0.13}\\
%     \bottomrule
% 	\end{tabular}

% \label{tab:rq3-1}
% \end{table}%

\begin{table}[t!]
	\centering
	\setlength{\tabcolsep}{2mm}
	\caption{RQ3: Average values of metrics at the final step  comparing between \approach$_{ran}$ and our method when using different pretrained language models. The best value of each performance indicator is in green.}

%all timesteps on 10 runs

% \resizebox{\textwidth}{!}{ % reSize the table
% \begin{tabular}{p{0.7cm}p{2cm}p{0.3cm}p{1.55cm}|p{0.3cm}p{1.55cm}|p{0.3cm}p{1.4cm}|p{0.3cm}p{1.4cm}|p{0.3cm}p{1.55cm}|p{0.3cm}p{1.4cm}}
% \toprule
% &
%   \multirow{2}{*}{\textbf{Model}} &
%   \multirow{2}{*}{\textbf{Approach}} &
%   \multicolumn{2}{c}{\textsc{\textbf{F1-score}}} &
%   \multicolumn{2}{c}{\textsc{\textbf{Accuracy}}} &
%   \multicolumn{2}{c}{\textsc{\textbf{Recall}}} &
%   \multicolumn{2}{c}{\textsc{\textbf{Precision}}} &
%   \multicolumn{2}{c}{\textsc{\textbf{Readability}}} &
%   \multicolumn{2}{c}{\textsc{\textbf{Identifiability}}}\\ \cline{4-14}

%  &
%  &
%    &
%   \textbf{$r$} &
%   \textbf{Average} &
%   \textbf{$r$} &
%   \textbf{Average} &
%   \textbf{$r$} &
%   \textbf{Average} &
%   \textbf{$r$} &
%   \textbf{Average} &
%   \textbf{$r$} &
%   \textbf{Average} &
%   \textbf{$r$} &
%   \textbf{Average} & \\ \hline
%  &
%   \texttt{\approach$_{ran}$}  &1&1&1&1&1&1&1&1&1&1&1&1\\
%  &
%   \texttt{\approach} &1&1&1&1&1&1&1&1&1&1&1&1 \\
%  &
%   \texttt{\approach$_{ran}$}  &1&1&1&1&1&1&1&1&1&1&1&1\\
% \multirow{-6}{*}{300}&
%   \texttt{\approach} &1&1&1&1&1&1&1&1&1&1&1&1 \\ 
% &
%   \texttt{\approach$_{ran}$}  &1&1&1&1&1&1&1&1&1&1&1&1\\
%  &
%   \texttt{\approach} &1&1&1&1&1&1&1&1&1&1&1&1 \\\hline
  
%  &
%   \texttt{\approach$_{ran}$}  &1&1&1&1&1&1&1&1&1&1&1&1\\
%  &
%   \texttt{\approach} &1&1&1&1&1&1&1&1&1&1&1&1 \\
% \multirow{-6}{*}{500} 
%  &
%   \texttt{\approach$_{ran}$}  &1&1&1&1&1&1&1&1&1&1&1&1\\
%  &
%   \texttt{\approach} &1&1&1&1&1&1&1&1&1&1&1&1 \\ 
% &
%   \texttt{\approach$_{ran}$}  &1&1&1&1&1&1&1&1&1&1&1&1\\
%  &
%   \texttt{\approach} &1&1&1&1&1&1&1&1&1&1&1&1 \\\hline
  
%  &
%   \texttt{\approach$_{ran}$}  &1&1&1&1&1&1&1&1&1&1&1&1\\
%  &
%   \texttt{\approach} &1&1&1&1&1&1&1&1&1&1&1&1 \\
% \multirow{-6}{*}{700} 
%  &
%   \texttt{\approach$_{ran}$}  &1&1&1&1&1&1&1&1&1&1&1&1\\
%  &
%   \texttt{\approach} &1&1&1&1&1&1&1&1&1&1&1&1 \\ 
% &
%   \texttt{\approach$_{ran}$}  &1&1&1&1&1&1&1&1&1&1&1&1\\
%  &
%   \texttt{\approach} &1&1&1&1&1&1&1&1&1&1&1&1 \\\hline

 
% \bottomrule
% \end{tabular}
% }

\resizebox{\textwidth}{!}{ % reSize the table
\begin{tabular}{p{1cm}p{1.5cm}p{2cm}p{0.3cm}p{1.55cm}|p{0.3cm}p{1.55cm}|p{0.3cm}p{1.4cm}|p{0.3cm}p{1.4cm}|p{0.3cm}p{1.55cm}|p{0.3cm}p{1.4cm}}
\toprule
 \multirow{2}{*}{\textbf{Size}} &\multirow{2}{*}{\textbf{Model}} &
  \multirow{2}{*}{\textbf{Approach}} &
  \multicolumn{2}{c}{\textsc{\textbf{F1-score}}} &
  \multicolumn{2}{c}{\textsc{\textbf{Accuracy}}} &
  \multicolumn{2}{c}{\textsc{\textbf{Recall}}} &
  \multicolumn{2}{c}{\textsc{\textbf{Precision}}} &
  \multicolumn{2}{c}{\textsc{\textbf{Readability}}} &
  \multicolumn{2}{c}{\textsc{\textbf{Identifiability}}}\\ \cline{4-15}

 &
 &
   &
  \textbf{$r$} &
  \textbf{Average} &
  \textbf{$r$} &
  \textbf{Average} &
  \textbf{$r$} &
  \textbf{Average} &
  \textbf{$r$} &
  \textbf{Average} &
  \textbf{$r$} &
  \textbf{Average} &
  \textbf{$r$} &
  \textbf{Average} \\ \hline
&&
  \texttt{\approach$_{ran}$}  &2&0.864&2&0.856&2&0.862&2&0.867&2&-49.548&2&0.053\\
&\multirow{-2}{*}{CodeBERT}&
  \texttt{\approach} &1&\textcolor{red}{0.875}&1&\textcolor{red}{0.866}&1&\textcolor{red}{0.881}&1&\textcolor{red}{0.87}&1&\textcolor{red}{-13.376}&1&\textcolor{red}{0.113}\\\cline{2-15}
&&
  \texttt{\approach$_{ran}$}  &2&0.867&2&0.857&2&0.87&2&0.863&2&-59.287&2&0.052\\  
&\multirow{-2}{*}{RoBERTa}&
  \texttt{\approach}  &1&\textcolor{red}{0.877}&1&\textcolor{red}{0.867}&1&\textcolor{red}{0.885}&1&\textcolor{red}{0.868}&1&\textcolor{red}{-6.543}&1&\textcolor{red}{0.101}\\\cline{2-15}
&&
  \texttt{\approach$_{ran}$} &2&0.879&2&0.871&2&0.883&1&\textcolor{red}{0.875}&2&-54.043&2&0.052\\
\multirow{-6}{*}{300} &\multirow{-2}{*}{RTA} &
  \texttt{\approach}  &1&\textcolor{red}{0.886}&1&\textcolor{red}{0.877}&1&\textcolor{red}{0.897}&2&0.874&1&\textcolor{red}{-2.207}&1&\textcolor{red}{0.108}\\ \hline
  
&&
  \texttt{\approach$_{ran}$}  &2&0.869&2&0.861&2&0.867&1&0.872&2&-47.712&2&0.054\\
&\multirow{-2}{*}{CodeBERT}&
  \texttt{\approach} &1&\textcolor{red}{0.88}&1&\textcolor{red}{0.871}&1&\textcolor{red}{0.887}&1&0.873&1&\textcolor{red}{-13.942}&1&\textcolor{red}{0.087}\\\cline{2-15}
&&
  \texttt{\approach$_{ran}$}  &2&0.87&2&0.861&2&0.869&2&0.87&2&-50.123&2&0.053\\  
&\multirow{-2}{*}{RoBERTa}&
  \texttt{\approach}  &1&\textcolor{red}{0.88}&1&\textcolor{red}{0.871}&1&\textcolor{red}{0.888}&1&\textcolor{red}{0.872}&1&\textcolor{red}{-11.754}&1&\textcolor{red}{0.103}\\\cline{2-15}
&&
  \texttt{\approach$_{ran}$} &2&0.884&2&0.875&2&0.89&1&0.878&2&-56.962&2&0.053\\
\multirow{-6}{*}{500} &\multirow{-2}{*}{RTA} &
  \texttt{\approach}  &1&\textcolor{red}{0.889}&1&\textcolor{red}{0.881}&1&\textcolor{red}{0.9}&1&0.879&1&\textcolor{red}{-11.52}&1&\textcolor{red}{0.129}\\ \hline

&&
  \texttt{\approach$_{ran}$}  &2&0.872&2&0.864&2&0.871&1&0.873&2&-57.184&2&0.052\\
&\multirow{-2}{*}{CodeBERT}&
  \texttt{\approach} &1&\textcolor{red}{0.882}&1&\textcolor{red}{0.873}&1&\textcolor{red}{0.889}&1&0.874&1&\textcolor{red}{-14.614}&1&\textcolor{red}{0.135}\\\cline{2-15}
&&
  \texttt{\approach$_{ran}$}  &2&0.871&2&0.862&2&0.872&2&0.87&2&-47.866&2&0.053\\  
&\multirow{-2}{*}{RoBERTa}&
  \texttt{\approach}  &1&\textcolor{red}{0.882}&1&\textcolor{red}{0.873}&1&\textcolor{red}{0.89}&1&\textcolor{red}{0.874}&1&\textcolor{red}{-15.198}&1&\textcolor{red}{0.117}\\\cline{2-15}
&&
  \texttt{\approach$_{ran}$} &2&0.884&2&0.876&2&0.889&1&0.879&2&-51.048&2&0.053\\
\multirow{-6}{*}{700} &\multirow{-2}{*}{RTA} &
  \texttt{\approach}  &1&\textcolor{red}{0.889}&1&\textcolor{red}{0.881}&1&\textcolor{red}{0.9}&1&0.879&1&\textcolor{red}{-14.105}&1&\textcolor{red}{0.13}\\\bottomrule
% &&
%   \texttt{\approach$_{ran}$}  &&0.853&&0.846&&0.841&&0.866&&-51.532&&0.053\\
% &\multirow{-2}{*}{CodeBERT}&
%   \texttt{\approach} &&0.864&&0.855&&0.863&&0.865&&-5.5&&0.165\\\cline{2-15}
% &&
%   \texttt{\approach$_{ran}$}  &&0.861&&0.852&&0.86&&0.861&&-50.017&&0.053\\
% &\multirow{-2}{*}{RoBERTa}&
%   \texttt{\approach}  &&0.868&&0.858&&0.874&&0.862&&-0.473&&0.157\\\cline{2-15}
% &&
%   \texttt{\approach$_{ran}$} &&0.875&&0.866&&0.88&&0.87&&-51.317&&0.053\\
% \multirow{-6}{*}{300} &\multirow{-2}{*}{RTA} &
%   \texttt{\approach}  &&0.88&&0.871&&0.891&&0.87&&-5.331&&0.156\\ \hline
  
% &&
%   \texttt{\approach$_{ran}$}  &&0.862&&0.854&&0.855&&0.869&&-52.605&&0.053\\
% &\multirow{-2}{*}{CodeBERT}&
%   \texttt{\approach} &&0.87&&0.861&&0.872&&0.868&&-14.026&&0.135\\\cline{2-15}
% &&
%   \texttt{\approach$_{ran}$}  &&0.865&&0.856&&0.865&&0.865&&-52.01&&0.053\\
% &\multirow{-2}{*}{RoBERTa}&
%   \texttt{\approach}  &&0.873&&0.864&&0.878&&0.867&&-12.0&&0.137\\\cline{2-15}
% &&
%   \texttt{\approach$_{ran}$} &&0.88&&0.871&&0.887&&0.873&&-51.033&&0.053\\
% \multirow{-6}{*}{500} &\multirow{-2}{*}{RTA} &
%   \texttt{\approach}  &&0.884&&0.875&&0.893&&0.875&&-16.241&&0.141\\ \hline

% &&
%   \texttt{\approach$_{ran}$}  &&0.866&&0.858&&0.862&&0.871&&-54.596&&0.052\\
% &\multirow{-2}{*}{CodeBERT}&
%   \texttt{\approach} &&0.875&&0.866&&0.878&&0.871&&-13.356&&0.126\\\cline{2-15}
% &&
%   \texttt{\approach$_{ran}$}  &&0.867&&0.859&&0.867&&0.868&&-52.139&&0.053\\ 
% &\multirow{-2}{*}{RoBERTa}&
%   \texttt{\approach}  &&0.875&&0.866&&0.882&&0.869&&-16.749&&0.137\\\cline{2-15}
% &&
%   \texttt{\approach$_{ran}$} &&0.881&&0.873&&0.887&&0.875&&-51.531&&0.053\\
% \multirow{-6}{*}{700} &\multirow{-2}{*}{RTA} &
%   \texttt{\approach}  &&0.885&&0.877&&0.894&&0.877&&-16.551&&0.139\\\bottomrule

\end{tabular}
}
\label{tab:rq3-1}
\end{table}%

==> tab/rq3_med.tex <==
\begin{table}[t!]
	\centering
	\setlength{\tabcolsep}{2mm}
	\caption{RQ3: Median values of metrics comparing between random and our method when using different pretrained language models. The best value of each performance indicator is in \textcolor{red}{RED}.}

	% \label{tab:rq3-1}%
	%\begin{threeparttable}
    \footnotesize
	\begin{tabular}{cccccccccc}\toprule
	\textbf{Step size}&\textbf{Model}&\textbf{Methods}\hspace{-0.5cm}&\textbf{F1-score}&\textbf{Accuracy}&\textbf{AUC}&\textbf{Recall}&\textbf{Precision}&\textbf{Readability}&\textbf{Identifiability}\\\midrule % times 27

   \multirow{6}{*}{300}&\multirow{2}{*}{CodeBERT}&Random&0.864&0.856&0.912&0.859&0.868&-47.225&0.052\\
   &&\approach&0.877&0.867&0.921&0.881&0.871&-1.993&0.101\\\cmidrule{2-10}
   &\multirow{2}{*}{RoBERTa}&Random&0.866&0.857&0.915&0.87&0.864&-55.797&0.052\\
   &&\approach&0.878&0.869&0.911&0.885&0.868&-8.267&0.099\\\cmidrule{2-10}
   &\multirow{2}{*}{RTA}&Random&0.88&0.871&0.916&0.883&0.876&-48.425&0.052\\
   &&\approach&0.886&0.877&0.926&0.898&0.876&-6.709&0.094\\
\midrule
   \multirow{6}{*}{500}&\multirow{2}{*}{CodeBERT}&Random&0.87&0.861&0.914&0.87&0.872&-48.459&0.053\\
   &&\approach&0.881&0.872&0.914&0.889&0.874&-15.562&0.083\\\cmidrule{2-10}
   &\multirow{2}{*}{RoBERTa}&Random&0.869&0.861&0.908&0.869&0.869&-48.517&0.053\\
   &&\approach&0.879&0.871&0.906&0.886&0.874&-10.104&0.093\\\cmidrule{2-10}
   &\multirow{2}{*}{RTA}&Random&0.883&0.876&0.923&0.89&0.878&-59.071&0.053\\
   &&\approach&0.889&0.881&0.922&0.901&0.879&-12.253&0.096\\
\midrule
   \multirow{6}{*}{700}&\multirow{2}{*}{CodeBERT}&Random&0.872&0.865&0.914&0.87&0.873&-56.881&0.052\\
   &&\approach&0.882&0.873&0.91&0.89&0.874&-6.647&0.121\\\cmidrule{2-10}
   &\multirow{2}{*}{RoBERTa}&Random&0.871&0.863&0.91&0.873&0.87&-47.229&0.053\\
   &&\approach&0.881&0.873&0.912&0.889&0.875&-13.273&0.101\\\cmidrule{2-10}
   &\multirow{2}{*}{RTA}&Random&0.884&0.876&0.923&0.888&0.879&-51.703&0.053\\
   &&\approach&0.888&0.88&0.913&0.898&0.881&-17.738&0.12\\
    \bottomrule
	\end{tabular}

\label{tab:rq3-1}
\end{table}%

==> tab/rq4.tex <==
\begin{table}[t!]
	\centering
        \footnotesize
	\setlength{\tabcolsep}{2mm}
	\caption{RQ4: Scott-Knott rank of metrics comparing~\approach with SOTA.. }
	\label{tab:rq1-1}%
	%\begin{threeparttable}
	\begin{tabular}{ccccccccc}\toprule
	\textbf{Step size}&\textbf{Methods/Metrics}\hspace{-0.5cm}&\textbf{F1-score}&\textbf{Accuracy}&\textbf{Recall}&\textbf{Precision}&\textbf{Readability}&\textbf{Identifiability}\\\midrule % times 27
  	
   \multirow{3}{*}{300} &Ours&1&1&2&1&1&1\\
   &Wu2021&5&5&1&5&3&2\\
   &Ge2021&2&2&5&2&2&2\\
   &Thung2015&3&3&3&4&4&3\\
   &Tu2022&4&4&4&3&5&4\\
\midrule
   \multirow{3}{*}{500} &Ours&1&1&2&1&1&1\\
   &Wu2021&5&5&1&5&3&2\\
   &Ge2021&2&2&5&2&2&2\\
   &Thung2015&3&3&3&4&4&3\\
   &Tu2022&4&4&4&3&5&4\\
\midrule
   \multirow{3}{*}{700} &Ours&1&1&2&1&1&1\\
   &Wu2021&5&5&1&5&3&2\\
   &Ge2021&2&2&5&2&2&2\\
   &Thung2015&3&3&3&4&4&3\\
   &Tu2022&4&4&4&3&5&4\\
	\end{tabular}	
\end{table}%

==> tab/rq4_med.tex <==
\begin{table}[t!]
	\centering
	\setlength{\tabcolsep}{2mm}
	\caption{RQ4: Median values of metrics comparing \approach with SOTA. The best value of each performance indicator is in \textcolor{red}{RED}.}
	\label{tab:rq4-1}%
	%\begin{threeparttable}
    \footnotesize
	\begin{tabular}{ccccccccc}\toprule
	\textbf{Step size}&\textbf{Methods/Metrics}\hspace{-0.5cm}&\textbf{F1-score}&\textbf{Accuracy}&\textbf{AUC}&\textbf{Recall}&\textbf{Precision}&\textbf{Readability}&\textbf{Identifiability}\\\midrule % times 27

 
    \multirow{5}{*}{300} 
    &Ours&\textcolor{red}{0.872}&\textcolor{red}{0.862}&\textcolor{red}{0.918}&0.877&\textcolor{red}{0.865}&\textcolor{red}{-3.491}&\textcolor{red}{0.098}\\
    &Wu2021&0.797&0.755&0.745&\textcolor{red}{0.909}&0.714&-82.543&0.052\\
    &Ge2021&0.825&0.814&0.813&0.827&0.824&-78.861&0.052\\
    &Thung2015&0.809&0.785&0.781&0.852&0.77&-82.436&0.052\\
    &Tu2022&0.805&0.786&0.783&0.839&0.777&-87.992&0.049\\
\midrule
   \multirow{5}{*}{500}
   &Ours&\textcolor{red}{0.878}&\textcolor{red}{0.87}&\textcolor{red}{0.916}&0.883&\textcolor{red}{0.872}&\textcolor{red}{-14.705}&\textcolor{red}{0.089}\\
    &Wu2021&0.806&0.767&0.757&\textcolor{red}{0.909}&0.724&-81.647&0.052\\
    &Ge2021&0.829&0.812&0.809&0.86&0.802&-78.976&0.052\\
    &Thung2015&0.825&0.807&0.803&0.86&0.795&-77.563&0.052\\
    &Tu2022&0.821&0.801&0.798&0.852&0.792&-88.342&0.053\\
\midrule
   \multirow{5}{*}{700}    
   &Ours&\textcolor{red}{0.879}&\textcolor{red}{0.87}&\textcolor{red}{0.919}&0.886&\textcolor{red}{0.873}&\textcolor{red}{-12.524}&\textcolor{red}{0.094}\\
    &Wu2021&0.805&0.766&0.756&\textcolor{red}{0.906}&0.724&-89.764&0.049\\
    &Ge2021&0.834&0.82&0.818&0.844&0.823&-89.183&0.049\\
    &Thung2015&0.829&0.812&0.809&0.857&0.805&-88.9&0.05\\
    &Tu2022&0.828&0.811&0.808&0.856&0.803&-92.466&0.051\\


    \bottomrule
	\end{tabular}
\end{table}%

==> tab/test.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% \begin{table*}[t!]
% \footnotesize
% \setlength{\tabcolsep}{1mm}
% \renewcommand\arraystretch{1.3}
\resizebox{\textwidth}{!}{ % reSize the table
\begin{tabular}{p{0.7cm}p{2cm}p{0.3cm}p{1.55cm}|p{0.3cm}p{1.55cm}|p{0.3cm}p{1.4cm}|p{0.3cm}p{1.4cm}|p{0.3cm}p{1.55cm}|p{0.3cm}p{1.4cm}}
\toprule
 &
  \multirow{2}{*}{\textbf{Approach}} &
  \multicolumn{2}{c}{\textsc{\textbf{F1-score}}} &
  \multicolumn{2}{c}{\textsc{\textbf{Accuracy}}} &
  \multicolumn{2}{c}{\textsc{\textbf{Recall}}} &
  \multicolumn{2}{c}{\textsc{\textbf{Precision}}} &
  \multicolumn{2}{c}{\textsc{\textbf{Readability}}} &
  \multicolumn{2}{c}{\textsc{\textbf{Identifiability}}}\\ \cline{3-14}

 &
   &
  \textbf{$r$} &
  \textbf{Med (IQR)} &
  \textbf{$r$} &
  \textbf{Med (IQR)} &
  \textbf{$r$} &
  \textbf{Med (IQR)} &
  \textbf{$r$} &
  \textbf{Med (IQR)} &
  \textbf{$r$} &
  \textbf{Med (IQR)} &
  \textbf{$r$} &
  \textbf{Med (IQR)} & \\ \hline
 &
  \texttt{Random}  &1&1&1&1&1&1&1&1&1&1&1&1\\
 &
  \texttt{Uncertainty} &1&1&1&1&1&1&1&1&1&1&1&1 \\
\multirow{-3}{*}{300} &
  \texttt{Effort} &1&1&1&1&1&1&1&1&1&1&1&1 \\  \hline
  
 &
  \texttt{Random}  &1&1&1&1&1&1&1&1&1&1&1&1\\
 &
  \texttt{Uncertainty} &1&1&1&1&1&1&1&1&1&1&1&1 \\
\multirow{-3}{*}{500} &
  \texttt{Effort} &1&1&1&1&1&1&1&1&1&1&1&1 \\  \hline
  
 &
  \texttt{Random}  &1&1&1&1&1&1&1&1&1&1&1&1\\
 &
  \texttt{Uncertainty} &1&1&1&1&1&1&1&1&1&1&1&1 \\
\multirow{-3}{*}{700} &
  \texttt{Effort} &1&1&1&1&1&1&1&1&1&1&1&1 \\ 

 
\bottomrule
\end{tabular}
}
% \end{table*}

